ConfLab: A Data Collection Concept, Dataset, and Benchmark for Machine Analysis of Free-Standing Social Interactions in the Wild

Recording the dynamics of unscripted human interactions in the wild is challenging due to the delicate trade-offs between several factors: participant privacy, ecological validity, data fidelity, and logistical overheads. To address these, following a 'datasets for the community by the community' ethos, we propose the Conference Living Lab (ConfLab): a new concept for multimodal multisensor data collection of in-the-wild free-standing social conversations. For the first instantiation of ConfLab described here, we organized a real-life professional networking event at a major international conference. Involving 48 conference attendees, the dataset captures a diverse mix of status, acquaintance, and networking motivations. Our capture setup improves upon the data fidelity of prior in-the-wild datasets while retaining privacy sensitivity: 8 videos (1920x1080, 60 fps) from a non-invasive overhead view, and custom wearable sensors with onboard recording of body motion (full 9-axis IMU), privacy-preserving low-frequency audio (1250 Hz), and Bluetooth-based proximity. Additionally, we developed custom solutions for distributed hardware synchronization at acquisition and time-efficient continuous annotation of body keypoints and actions at high sampling rates. Our benchmarks showcase some of the open research tasks related to in-the-wild privacy-preserving social data analysis: keypoints detection from overhead camera views, skeleton-based no-audio speaker detection, and F-formation detection.

==> scratch.tex <==
\subsection{Person and Keypoints Detection}
% [Ashraful] Define the tasks: includes person detection (bounding boxes) and keypoint detection.
% Object detection is the task of identifying the object of interests in the image in terms of object category and the precise bounding box of that object. We are interested particularly in person detection. A further extension of person detection is pose estimation, where the task is to localize human joints (elbows, wrists, etc.) in the image. Pose estimation is an important and often intermediate task towards understanding human actions and interactions in a scene (see Sec. \ref{sec:speaking-status}).

We developed a system for person detection (identifying bounding boxes) and pose estimation (localizing skeletal keypoints such as elbows, wrists, etc.). 
% Pose estimation is an important and often intermediate task towards understanding human actions and interactions in a scene (see Sec. \ref{sec:speaking-status}).
% \ash{Task definition: bounding box/ keypoint}
% \ash{baselines methods, short description of faster/mask-RCNN}
% \paragraph{Baseline methods} 
% Deep learning has revolutionized object detection and keypoint estimation starting with the development of the region-based convolutional neural network (RCNN) \cite{girshick2014richrcnn}. RCNN identifies a manageable number of rough object proposal boxes, which are then classified and regressed by a CNN to obtain an object label and box boundaries. Fast-RCNN \cite{girshick2015fastrcnn} and Faster-RCNN \cite{ren2016fasterrcnn} later built on its success by improving the speed and quality of object proposal generation. Mask-RCNN \cite{he2017maskrcnn} adopts the same approach, but adds an output branch to obtain object segmentations. The simplicity of Mask-RCNN enables its use for several tasks  with minimum architectural change producing competitive results on most benchmarks. We therefore adopt Mask-RCNN as our baseline method for person bounding box and keypoint detection tasks.
%We also perform experiments on bounding box detection task using faster-RCNN. 
%There are two dominant approaches for pose estimation. In the multi-step approach human bounding boxes are detected first and keypoints are regressed from the detected bounding boxes. In the end-to-end approach keypoints are directly predicted from input images. 
% \ash{Dataset description, data cleaning, how was train/val/test set constructed}
%\paragraph{Dataset preparation }

\paragraph{Predictions from pretrained state-of-the-art models}  Figure \ref{fig:pretrained_pred} shows predictions from state-of-the-art human keypoint estimation models, namely, RSN \cite{cai2020learningRSN}, MSPN\cite{li2019rethinkingmspn}, HigherHRNet \cite{Cheng_2020_CVPRhigherhrnet}, and HourglassAENet \cite{newell2017associative_posehglass}, for the testing images of the Conflab dataset. Note that RSN and MSPN are top-down networks, i.e., they require person bounding boxes to predict the keypoints in each bounding box. We use COCO pretrained faster-RCNN network for bounding box estimation. HigherHRNet and HourglassAENet are bottom-up models, i.e., they directly predict keypoints from the full image. We use publicly available COCO pretrained checkpoints for prediction. The results show that the \emph{state-of-the-arts 2D body keypoint detection models fail to capture the body keypoints in the Conflab dataset}. We infer that training on the dataset (e.g., COCO) that contains mostly side-view images does not work well in top-view images, for which Conflab dataset is important to the community.   

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/td/vid2-seg8-scaled-denoised_000082.jpg}
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/td/vid2-seg9-scaled-denoised_000059.jpg}
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/td/vid3-seg4-scaled-denoised_000863.jpg}
    
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/mspn/vid2-seg8-scaled-denoised_000082.jpg}
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/mspn/vid2-seg9-scaled-denoised_000027.jpg}
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/mspn/vid3-seg4-scaled-denoised_006082.jpg}
    
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/hr_pretrained/vid2-seg8-scaled-denoised_000082.jpg}
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/hr_pretrained/vid2-seg9-scaled-denoised_000027.jpg}
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/hr_pretrained/vid3-seg4-scaled-denoised_000494.jpg}
    
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/hglass/vid2-seg8-scaled-denoised_000082.jpg}
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/hglass/vid2-seg9-scaled-denoised_002403.jpg}
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/hglass/vid3-seg5-scaled-denoised_001567.jpg}
    
    
    \caption{Results from Pretrained keypoint detection models. From top to bottom - predictions from RSN \cite{cai2020learningRSN}, MSPN\cite{li2019rethinkingmspn}, HigherHRNet \cite{Cheng_2020_CVPRhigherhrnet}, and HourglassAENet \cite{newell2017associative_posehglass}. Results show that \emph{SOTA 2D body keypoint detection models fail to capture the body keypoints in the Conflab dataset}.}
    \label{fig:pretrained_pred}
\end{figure}

\paragraph{Experiments}
We used Mask-RCNN \cite{he2017maskrcnn} for both person detection and keypoint estimation tasks.  
Since keypoint annotations were made per camera, we used four of the overhead cameras for training and one for testing. The keypoint annotations contained some incorrectly labeled keypoints, a product of annotation errors like mis-assignment of participant IDs. We removed these using a threshold on the proximity to other keypoints of the same person. 
Missing keypoints were ignored during back-propagation. 
This resulted in a training set with 112k frames (1809k person instances) and a test set with 7k frames (158k person instances).
%Because of crowd-sourcing, there are many frames that contain erroneous person keypoints or keypoints that are incorrectly labeled. We first detect the valid keypoints based on proximity with the other keypoints of the same person, and the erroneous keypoints are not used for back-propagation during training. We also remove the entire frames if it contains more than 10\% null keypoints based on our proximity search. Table \ref{tab:dataset_des} shows number of frames, and number of person annotation and keypoints for all the number of frames, number of annotated persons, and valid annotated keypoints per person for both training and test set. 

% \begin{table}[!htbp]
%     \centering
%     \begin{tabular}{c c c c}
%     \toprule 
%         Set & Frames & Persons & {Keypoints per person} \\ 
%     \midrule
%     %   cam 2  & 63k & 608k & 30.6 \\
%     %   cam 4   & 27k & 553k & 33.9  \\
%     %   cam 6 & 42k & 50k & 32.2 \\
%     %   cam 8 & 49k &  \\
%     %   cam 10 & \\
         
%         training & 139k & 1588k & 32.03 \\
%         test & 42k & 50k & 32.17 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Data description.}
%     \label{tab:dataset_des}
% \end{table}


% \ash{baselines performance on bounding box and keypoint for different ResNet/FPN network}

% \subsubsection{Experiments}

% \paragraph{Implementation details}

We used the Detectron2 framework \cite{wu2019detectron2} to implement the baselines with ResNet-50 backbone. We resized the images to 960$\times$540, and applied random brightness and random horizontal flip augmentation. The learning rate was set to 0.02 and batch size to 4. We trained the models for 50k iterations. We use the COCO-pretrained weights for initialization. All hyper-parameters were chosen based on the performance on a separate hold-out camera chosen as validation set.

% \paragraph{Evaluation metrics} 
% We evaluated object detection performance using the standard evaluation metrics in the MS-COCO dataset paper \cite{lin2014microsoftcoco}. We report average precision (AP) for intersection over union (IoU) thresholds of 0.50 and 0.75, and the mean AP from an IoU range from 0.50 to 0.95 in 0.05 increments. For keypoint detection, IoU, undefined for single points, is replaced by object keypoint similarity (OKS) \cite{lin2014microsoftcoco} which measures Gaussian distance between two keypoints and returns a score between 0 and 1. AP$^\text{OKS}$ is a mean average precision for different OKS thresholds from 0.5 to 0.95. 

We evaluated object detection performance using the standard evaluation metrics in the MS-COCO dataset paper \cite{lin2014microsoftcoco}. We report average precision (AP) for intersection over union (IoU) thresholds of 0.50 and 0.75, and the mean AP from an IoU range from 0.50 to 0.95 in 0.05 increments. For keypoint detection, we use object keypoint similarity (OKS) \cite{lin2014microsoftcoco}. AP$^\text{OKS}$ is a mean average precision for different OKS thresholds from 0.5 to 0.95. 


% \paragraph{Results}

Table \ref{tab:mask_rcnn} summarizes our person detection and joint estimation results. Our baseline achieves 73.9 AP$_\text{50}$ in detection and 45.3 AP$^\text{OKS}_\text{50}$ in keypoint estimation using ResNet-50 backbone. Figure \ref{fig:det2pred} shows qualitative results from our finetuned network, which reveals that our finetuned network significantly improve the keypoint estimation performance for top-view images.

\begin{figure}[!tbp]
    \centering
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/det2_pretrained/vid2-seg8-scaled-denoised_006802.jpg}
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/det2_pretrained/vid2-seg9-scaled-denoised_000027.jpg}
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/det2_pretrained/vid3-seg1-scaled-denoised_000070.jpg}
    
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/det2/vid2-seg8-scaled-denoised_006802.jpg}
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/det2/vid2-seg9-scaled-denoised_000027.jpg}
    \includegraphics[width=0.3\linewidth]{imgs/keypoint/det2/vid3-seg1-scaled-denoised_000070.jpg}
    \caption{Results from (top) COCO pretrained Mask-RCNN model, (bottom) our Conflab finetuned Mask-RCNN model.}
    \label{fig:det2pred}
\end{figure}

% The low average AP$^\text{OKS}$ of 10.7 indicates that the estimated keypoints are imprecise. 

% The choice of backbone did not affect results significantly. Further experiments with Faster-RCNN (a detection-only model) and four different backbones (R50-C4, R101-C4, R50-FPN, and R101-FPN) revealed consistently better results for FPN backbones, with a best AP$_\text{50}$ of 51.49.

%Table \ref{tab:faster_rcnn} report the results for only person detection using Faster-RCNN network. We experiment with four different backbone - R50-C4, R101-C4, R50-FPN, and R101-FPN. We found that Feature Pyramid Network (FPN) \cite{lin2017featurefpn} backbones work better than C4 backbones for object detection. Surprisingly, larger backbone does not produce better detection results for our dataset. R50 backbones outperform R101 for both detection and keypoint estimation. This could be attributed to the small variability in frames between the same camera, such that larger backbone cannot benefit much from the dataset. 
%##################################################################################################
% \begin{table}[!htbp]
% \ra{1.2}
% \caption{\textbf{Mask-RCNN Results for person bounding box detection and keypoint estimation.} We find there is little performance gain for person detection with larger backbone, and performance degrades a little using larger backbone for keypoint estimation.}
% \centering
% \begin{adjustbox}{max width=\linewidth}
% \begin{tabular}{@{}lcccccc@{}} 
% \toprule
% \multirow{2}{*}{Model} &
%  \multicolumn{3}{c}{Person Detection} & \multicolumn{3}{c}{Keypoint Estimation} \\ \cmidrule{2-7} & AP$_\text{50}$ & AP & AP$_\text{75}$
% & AP$^\text{OKS}_\text{50}$ & AP$^\text{OKS}$ & AP$^\text{OKS}_\text{75}$ \\
% \midrule

% % R50-C4 \\
% % R101-C4 \\

% R50-FPN &  50.8 & 25.2 & 21.5 & 33.3 & 10.7 & 3.9\\
% R101-FPN & 50.9 & 25.6 & 24.2 & 31.5 & 9.8 & 3.2 \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \label{tab:mask_rcnn}
% \end{table}
%##################################################################################################
\begin{table}[!htb]
\begin{minipage}{.45\linewidth}

\ra{1.2}
\caption{Mask-RCNN Results for person bounding box detection and keypoint estimation.} 

% We find there is little performance gain for person detection with larger backbone, and performance degrades a little using larger backbone for keypoint estimation.}
\label{tab:mask_rcnn}
\centering
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}lcccccc@{}} 
\toprule
\multirow{2}{*}{Model} &
 \multicolumn{3}{c}{Person Detection} & \multicolumn{3}{c}{Keypoint Estimation} \\ \cmidrule{2-7} & AP$_\text{50}$ & AP & AP$_\text{75}$
& AP$^\text{OKS}_\text{50}$ & AP$^\text{OKS}$ & AP$^\text{OKS}_\text{75}$ \\
\midrule

% R50-C4 \\
% R101-C4 \\

% R50-FPN &  50.8 & 25.2 & 21.5 & 33.3 & 10.7 & 3.9\\
% R101-FPN & 50.9 & 25.6 & 24.2 & 31.5 & 9.8 & 3.2 \\

R50-FPN & 73.9 & 38.9 & 38.4 & 45.3 & 13.5 & 3.3  \\
% R101-FPN & 50.9 & 25.6 & 24.2 & 31.5 & 9.8 & 3.2 \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{minipage}\hfill
% \begin{minipage}{.45\linewidth}
%     \caption{Effect of training data size on keypoint estimation.}
%     \centering
%     \label{tab:abl_data_amount}
%     \begin{adjustbox}{max width=\linewidth}
%     \begin{tabular}{@{}lcc@{}}
%     \toprule
%       Train Camera  & AP$_\text{50}$ & AP$^\text{OKS}_\text{50}$ \\
%         %  &  \\
%     \midrule
%     cam 2 + cam 10 & 41.9 & 8.3 \\
%     cam 2 + cam 4 + cam 10 & 48.8 & 23.3 \\
%     cam 2 + cam 4 + cam 8 + cam 10 & 50.8 & 33.3 \\
%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
% \end{minipage}
\begin{minipage}{.45\linewidth}
    \caption{Effect of training data size on keypoint estimation.}
    \centering
    \label{tab:abl_n}
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{@{}lc@{}}
    % \toprule
    %   {Frames per video}  & AP$^\text{OKS}_\text{50}$ \\
    % \midrule
    % 100 & 29.0 \\
    % 200 & 35.9 \\
    % 500 & 39.0 \\
    % 1000 & 44.5 \\
    % Full & 45.3 \\
    \toprule
       {\% of training samples}  & AP$^\text{OKS}_\text{50}$ \\
    \midrule
    1.6\% & 29.0 \\
    3.2\% & 35.9 \\
    8\% & 39.0 \\
    16\% & 44.5 \\
    100\% & 45.3 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{minipage}
\end{table}


%##################################################################################################
% \begin{table}[!htbp]
% \centering
% \begin{tabular}{l  l l l } 
% \toprule
% model & AP$_\text{50}$ & AP & AP$_\text{75}$ \\
% \midrule

% R50-C4 & 44.27 & 21.91 & 18.05 \\
% R101-C4 & 43.37 & 21.62 & 19.50 \\

% R50-FPN & 51.49 & 25.12 & 21.98 \\
% R101-FPN & 44.29 & 23.62 & 22.47 \\

% \bottomrule
% \end{tabular}
% \caption{Person bounding box detection results using faster RCNN.}
% % }
% \label{tab:faster_rcnn}
% \end{table}
%##################################################################################################

% \subsubsection{Analysis}

% \paragraph{Effect of amount of labeled data}

% \ash{Analysis: effect of amount of labeled data}

%\paragraph{Effect of size of training data}

We performed an analysis to show the effect of training data on the final evaluation.
In Table \ref{tab:abl_n}, we show results when varying percentage of training samples are used for training. Note that we use all the cameras for training, just the number of frames for each camera are varied, where we have 16 training cameras. The results show that we can achieve saturation in performance at 16\% training samples. However, here, we are still using all the individual cameras just the number of frames for each camera are varied. Next, we show experiments on training the network on camera 2, camera 2 and 4, and all cameras   in  Table \ref{tab:abl_data_amount}, We evaluate the same testing images consisting of one camera view (camera 6). There is a big performance improvement when we add multiple camera views in the training set. ConfLab features high person scene density (15 on average per camera view) which may be a useful resource for developing overhead keypoint estimation. 

\begin{table}[!t]
\caption{Effect of training data size on keypoint estimation.}
    \centering
    \begin{tabular}{@{}lcc@{}}
    \toprule
      Train Camera & \#(training samples) & AP$^\text{OKS}_\text{50}$ \\
        %  &  \\
    \midrule
    cam 2 & 34k & 8.6 \\
    cam 2 + cam 4 & 69k & 31.1 \\
    cam 2 + cam 4 + cam 8 & 112k & 45.3 \\
    \bottomrule
    \end{tabular}
    \label{tab:abl_data_amount}
\end{table}


% \paragraph{Effect of number of keypoints}

% \begin{table}[!htbp]
%     \centering
%     \begin{tabular}{c|c c}
%     \toprule
%       Keypoints & AP$_\text{50}$ & AP$^\text{OKS}_\text{50}$ \\
%          &  \\
%     \midrule
%       \\
%     \\
%      \\
%     \bottomrule
%     \end{tabular}
%     \caption{\small Effect of amount of dataset for keypoint estimation.}
%     \label{tab:abl_diff_kp}
% \end{table}

% \ash{Analysis: Effect of number of keypoints}

% \paragraph{Qualitative examples}
% \ash{Qualitative example}

% \paragraph{Characterising performance vs amount of labeled data}
% Includes a figure and, or table 
% \paragraph{Characterising performance vs keypoints subgroups}
% Includes a figure and, or table


%%%%%%%%%%%%%%%%%%%%%%%%% PROTOCOL
% Participants who wanted to leave the event were again directed to the registration desk and their Midges were collected and turned off. After one hour of interaction, a team member announced the end of the event and remaining participants left the recording area and dropped off their Midges. 
% Approximately fifteen to twenty minutes before the event's announced starting time, all Midge s were turned on and put on the top of the registration desk. When participants first arrived to the recording area, they were greeted by the team and volunteers from the conference organization and directed to the registration desk. Team members present in the registration desk first fitted the participant with a Midge. The ID of this Midge also acted as the participant's identifier. Then, another team member took a picture of the participant while making sure both the face of the participant and the ID on the Midge were visible. After this initial welcome and wearable sensor fitting, participants were directed to the interaction area which was recorded by multiple cameras. After all participants were fitted with Midge s, one member of the team gave an opening speech which explained the event briefly. This speech ended with the pop of a balloon which signified the start of the event. During the event, participants mingled freely without any constraints, other than staying in the recording area. Participants who wanted to leave the event were again directed to the registration desk and their Midge s were collected and turned off. After approximately one hour after the start of the event, a team member announced the end of the event and participants left the recording area and dropped off their Midge s. 

==> tab-summary-conflab.tex <==
% \begin{table}[h!]
% \centering
% \begin{tabularx}{\linewidth}{ | X | X | X | }
%  \hline 
%  Input & Modality / annotation & Detail \\ 
%  \hline
%  \multirow{2}{*}{Cameras} & Overhead & 9, equally spaced \\ 
%  \cline{2-3}
%  & Elevated side-view & 4, one on each corner \\ 
%  \hline
%  \multirow{3}{*}{Wearable sensors} & IMU & Chest-worn IMU @ 60Hz \\ 
%  \cline{2-3}
%  & Low-frequency audio & Mono @ 1200Hz\\ 
%  \cline{2-3}
%  & Proximity & TODO \\ 
%  \hline
%  \multirow{3}{*}{Manual annotations} & Body pose & For 5 cameras and 16 min \\ 
%  \cline{2-3}
%  & Speaking status & For 16 min ? \\ 
%  \cline{2-3}
%  & F-formations & TODO \\ 
%  \hline
% \end{tabularx}
% \caption{Summary of modalities and annotations in the \ConfLab dataset.}
% \end{table}

% \begin{table}[]
% \caption{Capture setup and annotations in the \ConfLab dataset.}
% \label{tab:summary-conflab}
% \begin{tabular}{@{}ll@{}}
% \toprule
% \textbf{Modality} & \textbf{Details}          \\ \midrule
% \textbf{Cameras}               &                          \\
% \hspace{2mm}Overhead                       & 9, 1~m intervals       \\
% \hspace{2mm}Elevated side-view             & 4, one at each corner    \\ \midrule
% \textbf{Wearable Sensors}      &                          \\
% \hspace{2mm}IMU                            & Chest-worn, 60Hz    \\
% \hspace{2mm}Low-frequency audio            & Mono, 1200Hz            \\
% \hspace{2mm}Proximity                      & TODO                     \\ \midrule
% \textbf{Manual Annotations}    &                          \\
% \hspace{2mm}Body pose                      & 5 cameras, 16 min \\
% \hspace{2mm}Speaking status                & 16 min ?             \\
% \hspace{2mm}Conversation groups            & TODO                     \\ \bottomrule
% \end{tabular}
% \end{table}
